Deterministic Real-Time Tree-Walking-Storage Automata

We study deterministic tree-walking-storage automata, which are finite-state devices equipped with a tree-like storage. These automata are generalized stack automata, where the linear stack storage is replaced by a non-linear tree-like stack. Therefore, tree-walking-storage automata have the ability to explore the interior of the tree storage without altering the contents, with the possible moves of the tree pointer corresponding to those of tree-walking automata. In addition, a tree-walking-storage automaton can append (push) non-existent descendants to a tree node and remove (pop) leaves from the tree. Here we are particularly considering the capacities of deterministic tree-walking-storage automata working in real time. It is shown that even the non-erasing variant can accept rather complicated unary languages as, for example, the language of words whose lengths are powers of two, or the language of words whose lengths are Fibonacci numbers. Comparing the computational capacities with automata from the classical automata hierarchy, we derive that the families of languages accepted by real-time deterministic (non-erasing) tree-walking-storage automata is located between the regular and the deterministic context-sensitive languages. There is a context-free language that is not accepted by any real-time deterministic tree-walking-storage automaton. On the other hand, these devices accept a unary language in non-erasing mode that cannot be accepted by any classical stack automaton, even in erasing mode and arbitrary time. Basic closure properties of the induced families of languages are shown. In particular, we consider Boolean operations (complementation, union, intersection) and AFL operations (union, intersection with regular languages, homomorphism, inverse homomorphism, concatenation, iteration). It turns out that the two families in question have the same properties and, in particular, share all but one of these closure properties with the important family of deterministic context-free languages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{Rudolf Freund, Benedek Nagy (Eds.): 13th International Workshop on \\ Non-Classical Models of Automata and Applications (NCMA 2023)\\
EPTCS 388, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.388.7}{10.4204/EPTCS.388.7}}
\pdfoutput=1

